Evaluating Adversarial Robustness of Low dose CT Recovery

Low dose computed tomography (CT) acquisition using reduced radiation or sparse angle measurements is recommended to decrease the harmful effects of X-ray radiation. Recent works successfully apply deep networks to the problem of low dose CT recovery on bench-mark datasets. However, their robustness needs a thorough evaluation before use in clinical settings. In this work, we evaluate the robustness of different deep learning approaches and classical methods for CT recovery. We show that deep networks, including model-based networks encouraging data consistency, are more susceptible to untargeted attacks. Surprisingly, we observe that data consistency is not heavily affected even for these poor quality reconstructions, motivating the need for better regularization for the networks. We demonstrate the feasibility of universal attacks and study attack transferability across different methods. We analyze robustness to attacks causing localized changes in clinically relevant regions. Both classical approaches and deep networks are affected by such attacks leading to changes in the visual appearance of localized lesions, for extremely small perturbations. As the resulting reconstructions have high data consistency with the original measurements, these localized attacks can be used to explore the solution space of the CT recovery problem.

==> hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}

==> tab_untargeted.tex <==
\begin{table}[htb]
    \centering
\resizebox{\linewidth}{!}{\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{Method}&\multicolumn{4}{c}{LoDoPaB}&\multicolumn{4}{c}{LoDoPaB\_200}\\
&clean&$\epsilon=0.01$&$\epsilon=0.025$&$\epsilon=0.05$&clean&$\epsilon=0.01$&$\epsilon=0.025$&$\epsilon=0.05$\\
    \midrule
   FBP&30.52/ 0.737& 24.99/0.432&18.44/ 0.182&12.78/0.069&28.45/0.645  & 25.16/0.453& 19.58/0.223 & 14.17/0.091\\
   TV\\
   FBP-Unet&35.84/0.844 & 18.14/0.271&12.04/0.09&7.23/0.03&33.89/0.810 & 19.18/0.375 & 12.66/0.113 & 8.30/0.036\\
   iRadonMap\\
   LearnedPD&36.12/ 0.850&9.32/0.153&3.51/0.031& 0.355/0.008&33.98/0.813&17.61/0.405&10.49/0.147&5.95/0.051\\
   LearnedGD&34.88/0.824&20.92/0.499&13.71/0.285& 8.53/0.173&32.78/0.787&22.36/0.587&15.59/0.421&10.94/0.302\\
    \bottomrule
    \end{tabular}}
    \caption{Comparison of robustness to untargeted attacks on different CT reconstruction methods when sampling 513 and 200 projection beams out of 1000 parallel beams using 20 attack iterations. Average PSNR/SSIM values on LoDoPAB testset are reported.}
    \label{tab:untargetted_full}
\end{table}
\vspace{-1em}
